An implicit, conservative electrostatic particle-in-cell algorithm for paraxial magnetic nozzles

An electrostatic, implicit particle-in-cell (PIC) model for collisionless, fully magnetized, paraxial plasma expansions in a magnetic nozzle is introduced with exact charge, energy, and magnetic moment conservation properties. The approach is adaptive in configuration space by the use of mapped meshes, and exploits the strict conservation of the magnetic moment to reduce the dimensionality of velocity space. A new particle integrator is implemented, which allows for particle substepping without the need to stop particle motion at every cell for charge conservation. Particle suborbits are determined from accuracy considerations, and are allowed to span multiple cells. Novel particle injection and expansion-to-infinity boundary conditions are developed, including a control loop to prevent the formation of spurious sheaths at the edges of the domain. The algorithm is verified in a periodic magnetic mirror configuration, a uniform plasma test case (to test particle injection), and a propulsive magnetic nozzle. The algorithm's computational complexity is shown to scale favorably with timestep, and linearly with the number of particles and mesh cells (unlike earlier implicit PIC implementations, which scaled quadratically with the number of mesh cells in one dimension). Numerical experiments demonstrate that the proposed algorithm outperforms both explicit PIC and semi-Lagrangian Vlasov codes by more than an order of magnitude.

==> letter.tex <==
Please find attached an electronic copy of the manuscript “An implicit, conservative electrostatic particle-in-cell algorithm for paraxial magnetic nozzles”, by Pedro Jiménez, Luis Chacon, and Mario Merino which we submit for publication in your esteemed journal. 

This work presents a state-of-the-art Implicit Particle in Cell (PIC) algorithm for the study of magnetic nozzles (MN). Among the main novelties you may find the introduction of new boundary conditions that enable the simulation of an infinite expansion in a finite domain and the generalization of a faster and more scalable particle mover in mapped geometries that builds on, and we believe surpasses, algorithms presented in previous implicit PIC studies. The algorithm is thoroughly verified with two simplified configurations, showing the advertised conservation properties, and a MN case compared to previous literature. We also study the scaling of computational complexity with different numerical parameters and present an estimate of the algorithm’s performance gain compared to conventional simulation tools. 

We believe that this manuscript will be of great interest to JCP readers working in fields related like plasma simulation and electric propulsion and that it presents a combination of algorithmic advances and physics simulation that is perfectly suited for the journal. We look forward to hearing from you. The manuscript is neither copyrighted, classified, published, nor being considered for publication elsewhere. A single PDF file with texts and figures is sent. Separate text and figure files will be sent upon request. 


==> recortes.tex <==
Observe that the axial motion of each particle is determined by the effective potential $U_{\mathrm{eff},s}$ defined in \cite{mart15a} as 
%
\begin{align}\label{eq:effpot}
U_{\mathrm{eff},s}(z,t; \tilde{\mu})
= \frac{q_s}{m_s}\phi + \tilde{\mu} B,
\end{align}
%
for $s=i,e$. 
While $\phi$ is  monotonically decreasing along the MN in the cases of interest,
$U_{\mathrm{eff},s}$ is generally nonmonotonic, at least for some $\bar \mu_s$. 
This subdivides each species into free-streaming, reflected, and trapped subpopulations of particles, depending on 
the connectivity of their trajectories with the upstream plasma source 
and infinity downstream \cite{mart15a, ahed20a, meri21a}. This connectivity is dictated by their mechanical energy and magnetic moment, and the potential barriers in $U_{\mathrm{eff},s}$.
Naturally, in a time-dependent context with changing $\phi$, the boundaries between these sub-populations are dynamic; as a possibility, initially free particles may become trapped during the transient setup of the plasma beam \cite{sanc18b}, and vice versa, as $\phi$ evolves and their mechanical energy changes. Finally, we note that other mechanisms outside of the present model, including collisions, can lead to the exchange of particles between the different subpopulations also in the steady state \cite{zhou21a}.


-------------------------





The electron's instantaneous specific energy is
%
\begin{equation}
    E_p = -\frac{e\phi_p}{m_e} + 1/2v_p^2 + \Tilde{\mu}_pB_p,
\end{equation}
%
where $\phi_p$ and $B_p$ are evaluated at the current position of the particle. At steady state, each particle feels an effective potential energy map given by \eqref{eq:effpot}\lc{missing cross ref.}, for electrons,
%
\begin{equation}
    U_{eff,e}(z)=-\frac{e\phi}{m_e} + \Tilde{\mu}_pB.
\end{equation}
%
The potential energy is not known outside the domain, but it suffices to assume that it increases monotonically such that $U_{eff,e}(z=\infty)=-e\phi_\infty/m_e$. Consequently, we can classify electrons according to the following criteria,
\begin{enumerate}[label=\arabic*.]
    \item $E_p>-e\phi_\infty$ : This is a free electron, it will travel to infinity.
    \item $E_p<-e\phi_\infty$: The electron will be reflected back by the decreasing potential. 
    \begin{enumerate}[label*=\arabic*.]
        \item $E_p>U_{eff,e}(z)\;\forall\; z<z_p$: It will be reflected back to the source.
        \item $E_p<U_{eff,e}(z)\;\text{for any}\; z<z_p$: The electron is located at a potential well and has no energy to escape so it bounces between the two locations. We refer to this kind of electron as doubly trapped.
    \end{enumerate}
\end{enumerate} 



-------






%% MAGNETIC moment conservation
Expressing $\dot{v}_\perp$ in terms of $\mu$ and its derivatives, conservation of magnetic moment $\mu = m v_{\perp}^2/2B$ can be derived from the last equation,
%
\begin{equation}
    \begin{aligned}
        &v_{\perp}^2  = 2B\mu/m, \\
        &m \frac{\mathrm{d} v_{\perp}}{\mathrm{d} t}=\frac{1}{v_{\perp}}\left(\mu \frac{\mathrm{d} B}{d t}+B \frac{\mathrm{d} \mu}{\mathrm{d} t}\right),
    \end{aligned}
\end{equation}
%
where the total derivative of the magnetic field as the particle streams in $z$ is
%
\begin{equation}
    \frac{d B}{d t}=\frac{\partial B}{\partial t}+v_{\|} \frac{\partial B}{\partial z}=v_{\|} \frac{\mathrm{d} B}{\mathrm{~d} z},
\end{equation}
%
plugging into \eqref{eq:vper}
%
\begin{equation}
    \frac{1}{v_{\perp}}\left(\mu v_{\|} \frac{\mathrm{d} B}{\mathrm{~d} z}+B \frac{\mathrm{d} \mu}{\mathrm{d} t}\right)=\frac{m}{2 B} \frac{d B}{d z} v_{\perp} v_{\|}
\end{equation}
%
reintroducing the definition $\mu$, it can be observed that the first left-hand side term and the right-hand side one cancel out leaving, 
%
\begin{equation}
    \frac{B}{v_{\perp}} \frac{\mathrm{d} \mu}{\mathrm{d}t}=0,
\end{equation}
%
which in general implies $\dot{\mu} = 0$. From this point $\mu$ is considered constant for each particle. We write \eqref{eq:vpar} as

\appendix
\section{Implicit PIC performance gain}

\mmm{Lo reviso y si puedo lo integro arriba}

As mentioned above, our simulations are about 25 times faster than \cite{sanc18b} running on similar machines. That work, however, employed a Vlasov Semi-Langrangian discretization that is known to be less noisy but considerably more expensive than particle codes. It is possible to use our parametric studies on the computational times with different numerical parameters to obtain an estimate of the time that it would take for a similarly optimized explicit PIC (ePIC) code to run the same nozzle simulations. In doing so, we aim at quantifying a lower bound for the potential gain in the implementation of implicit codes.

Our mesh selection is constrained by the need to set quite small cells at the entrance (in the order of the Debye length). Despite the quasineutrality control imposed thereby, spurious oscillations were significantly reduced upon mesh refinement in the convergent part of the nozzle. This imposes a heavy burden on our simulations because, provided a statistically significant minimum number of particles per cell, the total number of particles in steady state grows inversely proportional to the cell size at the entrance. Note that this problem could be solved with population control strategies in future studies. Given the large $\Delta t$ employed in our simulations, such algorithms would probably represent only a very small fraction of the total computation time and help unlock the full potential of the iPIC coming from the reduction in the total number of particles that derives from its capability to use over-Debye length meshes. 

Without population control in either scenario, we will assume that the steady-state number of particles would be equal in an explicit simulation. On the other hand, the ePIC requirement to resolve the local Debye length in the rest of the domain (Birdsall sets this limit at $ \Delta z<\pi\lambda_D$ \cite{BIRD91}) implies a considerably finer mesh than ours elsewhere but in the comparable convergent region. Nevertheless, we observe that the cost of the field solver is secondary to the particle mover and disregard this increase (for explicit simulations) on the number of cells for our estimation. Notice that while this is true in 1D, the solution of the field in higher dimensions tends to represent a larger fraction of the computational time; in such a case the iPIC \pjj{si os gusta lo defino en la introducción} benefits greatly from a coarser mesh, even in the unlikely case that the total number of particles remained fixed.

Finally, we can study the gain that comes from a large $\Delta t$. When the timestep is small, the JFNK solver can achieve convergence in a few iterations (in the limiting case 1 iteration). Additionally, the particles tend to perform one unique suborbit per timestep. Thus, the cost of iteration in this limit is approximately independent of the timestep and the total computational time scales as $T_c \propto 1/\Delta t$. This is shown in Figure \ref{fig:times} left; notice how the measured $T_c$ curve approaches the limit for small enough $\Delta t$. For larger time steps, this relation no longer holds because both the mover performs more suborbits per particle and the solver needs more iterations to converge the electrostatic field.  The new segment-based mover, which allows particles to cross several cells in a single suborbit, improves performance by making the numerical curve approach closer to the small timestep limit. 

As a conservative approximation to the behavior of an explicit equivalent simulation, we can extrapolate a straight line in $T_c$ vs. $1/\Delta t$ keeping the slope found for our two smallest $\Delta t$ (notice that this underestimates the total times for $\Delta t < \Delta t_1)$:

\begin{equation}
T_c(\Delta t)=T_1+\frac{T_{c,1}-T_{c,2}}{1/\Delta t_1-1/\Delta t_2}(1/\Delta t-1/\Delta t_1)
\end{equation}

We find, for a typical explicit timestep of 0.1 $(\omega_{pe}) ^{-1}$, an estimate time of about 125000 s. Although costly weighting and interpolation operations and memory fetches are equivalent, we can apply a reduction factor of 2 to this number to account for the increase in floating-point operations of the implicit mover compared to the simple explicit mover. Compared to our nominal simulation with $T_c = 7200$ s, the result is a lower bound for the reduction in computational time of about 8.5. 

\mmm{me queda revisar esto y conclusiones} \lc{Necesita discusi\'on, enfoque, y reducci\'on. Pedro, los gr\'aficos en Fig. 10 son v\'alidos, pero hay que destilar los mensajes importantes. }\pjj{Es que veo que si no explico ciertas cosas se queda coja la discusión o no se justifica la estimación. Voy a pensar como limpiarlo}

Simulation Case B was run with different numbers of particles per cell and integration timesteps, leading to the results reported in Figure \ref{fig:convergence}.
We measure the error as a root mean square deviation (RMSD) in the steady state $\phi$ and $T_{e\|}$ spatial profiles with respect to the reference simulation B1.
With comparable numerical parameters, similar computation times and errors were observed in a less detailed analysis of Case A. This is reflected in the almost perfect match of A and B profiles upstream of the exit sheath. 

The nominal solution shows excellent convergence, with a root mean square difference below $0.004$ $T_e^*/e$ on the $\phi$ map and below $0.0075$ $T_e^*$ on all temperatures. While the results above are accumulated in a 500 $(\omega_{pe})^{-1}$, we observe some steady-state oscillations in the instantaneous potential; these have a standard deviation around the mean potential value of $0.11$ $T_e^*/e$ for case B and $0.03$ $T_e^*/e$ for the fine case B1. The noise is most likely related to the interaction of the dynamic boundary condition and the injection and reflection control algorithms, but does not have any visible effect on the averaged results. Consistent with the correct functioning of the suborbiting integration algorithm, variations in $\Delta t$ do not affect the error reported above in any clear trend, but do lead to an increase in steady-state oscillations (up to a standard deviation of $0.17$ $T_e^*/e$ in $\phi_\infty$ for $\Delta t = 10 (\omega_{pe})^{-1}$). In contrast, increasing the number of particles per cell $N_p$ does come with a remarkable reduction in both the RMSD errors and noise. Correlation with the Monte Carlo error $1/\sqrt{N_p}$ is not apparent in our results. \lc{Yo creo que si; dib\'ujalas en escala logar\'itmica a ver}\pjj{No parece claro, probablemente entran en juego otros factores, te he subido a figures la misma con 1/sqrt(Np). Se puede quitar la frase para no despistar}

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=\textwidth]{figures/convergence.png}
%     \caption{Root mean square deviation (RMSD) to the finest simulation (B1) potential (\mycirc $T_e^*/e$ units) and temperature (\mysquare $T_e^*$ units) and total computational time as a function of the integration timestep $\Delta t$ (left) and the number of particles in the first cell $N_p$ (right).}
%     \label{fig:convergence}
% \end{figure}

The computational times using 20 threads on an Intel Xeon (R) 4316 machine are reported in the bottom row of Figure \ref{fig:convergence}. The behavior as a function of the timestep is governed by various effects. On the one hand, the increase with $\Delta t$ in the number of suborbits per particle and the need for more JFNK iterations until convergence make each integration step longer. On the other hand, there is an inverse proportional relation between $\Delta t$ and the total number of steps. Consistent with the balance between these effects, we observe a saturation in computational times for $\Delta t > 10 (\omega_{pe})^{-1}$, a behavior anticipated by Chen et al. in early implicit PIC studies \cite{chen14}. \pjj{Another key factor that favors implicit PIC performance is the improvement in CPU utilization that comes from the reduction in mem.    ory fetches over floating point operations the larger the $\Delta t$. After profiling, we estimate a parallel efficiency of about $75\%$ for $\Delta t = 10$ that drops to $\sim54\%$ for $\Delta t =1.0$} 

\pjj{Luego lo vemos}. 

Finally, the CPU wall time scales almost linearly with the number of particles. This is also true for mesh size (not displayed here) as long as we keep the number of particles per cell constant. The increase in computational time for the finer mesh cases is driven by the change in total particle count; on the other hand, field solver times seem to remain negligible compared to the integration of particle orbits.

Our nominal simulation runs in about 2 hours. It is interesting to perform a back-of-the-envelope estimation on the speedup of the implicit algorithm compared to conventional kinetic codes. Explicit PIC solvers are constrained to resolve the local Debye length everywhere in the domain in order to avoid finite grid instabilities and numerical heating. For low order explicit PIC, Birdsall sets the limit cell size at $\Delta z < \pi \lambda_D$ \cite{BIRD94}. Sanchez et al. \cite{sanc18b} used 1501 nodes in the spatial discretization with their Eulerian solver, a node density which may be an overkill for standard PIC solvers. Without further evidence, we think that a mesh of about 750 cells would probably be sufficient in such a case. If the same number of particles per cell were kept for acceptable statistics, and neglecting any overhead associated with the field solver and weighting procedures, we can assume $t_{tot}\propto n_z$. This introduces a factor $\sim\times6$ upon changing from our 128 cell mesh to the explicit one.  

When the timestep is small, the JFNK solver can achieve convergence in a few iterations (in the limiting case 1 iteration). Additionally, the particles tend to perform one unique suborbit per timestep. Thus, the cost of iteration in this limit is approximately independent of the timestep and the total computational time scales as $t_{tot} \propto 1/\Delta t$. This is shown in Figure \ref{fig:convergence} (bottom,left); note how the measured $t_{tot}$ curve approaches the limit for small enough $\Delta t$. At our smallest $\Delta t$, we still observe 4 non-linear function evaluations ($N_{FE}$ or calls to the particle mover) consistently throughout the duration of simulation. Extending the limit curve to a typical explicit integration step of 0.1 $(\omega_{pe}^*)^{-1}$, and applying the $1/N_{FE}$ factor, the estimated $t_{tot}$ is $\sim\times 6$ the nominal one.
